Imagined versus Remembered Stories: Quantifying Differences in Narrative Flow

Lifelong experiences and learned knowledge lead to shared expectations about how common situations tend to unfold. Such knowledge of narrative event flow enables people to weave together a story. However, comparable computational tools to evaluate the flow of events in narratives are limited. We quantify the differences between autobiographical and imagined stories by introducing sequentiality, a measure of narrative flow of events, drawing probabilistic inferences from a cutting-edge large language model (GPT-3). Sequentiality captures the flow of a narrative by comparing the probability of a sentence with and without its preceding story context. We applied our measure to study thousands of diary-like stories, collected from crowdworkers about either a recent remembered experience or an imagined story on the same topic. The results show that imagined stories have higher sequentiality than autobiographical stories and that the sequentiality of autobiographical stories increases when the memories are retold several months later. In pursuit of deeper understandings of how sequentiality measures the flow of narratives, we explore proportions of major and minor events in story sentences, as annotated by crowdworkers. We find that lower sequentiality is associated with higher proportions of major events. The methods and results highlight opportunities to use cutting-edge computational analyses, such as sequentiality, on large corpora of matched imagined and autobiographical stories to investigate the influences of memory and reasoning on language generation processes.

==> figures/contextuality-density.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{graphics/hcV2_recImgAgn_summaryCtx_xent_linearity_bw.pdf}
    \caption{Caption}
    \label{fig:hc-contextuality}
\end{figure}

==> figures/suprisingness-with-context.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{graphics/hcV2_gptPplx_xent_summaryCtx_allHistSizes_v2.pdf}
    \caption{Caption}
    \label{fig:hc-surp-history}
\end{figure}

==> sections/_0-significance.tex <==

% \maarteninline{Exactly 120 words!}
\newText{
We explore the open question of analyzing the differences in narrative flow of stories generated from memory versus via imagination.
We introduce \bagChainName, a computational measure of narrative flow of events that compares the influence of preceding sentences versus story topic on story sentences, using a cutting-edge large language model (GPT-3).
Applying \bagChainName to thousands of imagined and recalled stories, we find that narrative flow relies more on preceding sentences in imagined stories, versus more on story topic for recalled stories.
% We additionally find that the flow of autobiographical narratives become more similar to imagined stories when retold several months later.
Shedding light onto our novel computational measure, we additionally uncover a link between events perceived as salient and \bagChainName.
The methods and results open a window into the distinct cognitive processes harnessed with recalling experiences versus imagining them. 
}



==> tables/nlp-corpora.tex <==
\begin{table}[h]
    \centering
    \caption{Effect sizes of our linearity measure on various corpora, along with the direction of the effect (opposite direction in parentheses).
    Effects are significant at $^{***}$:$p<0.001$ and $^{**}$:$p<0.05$.}
    \begin{tabular}{lr@{}lc}
        \toprule
        corpus & \multicolumn{2}{c}{effect size}  & direction \\ \midrule
        Hippocorpus & 0.52 & $^{***}$ & imagined (vs. recalled) \\
        DeceptiveReviews & 0.14 & $^{**}$ &  deceptive (vs. real) \\
        StoriesInTheWild & 0.82 & $^{***}$ & in full (vs. sequentially) \\ \bottomrule
    \end{tabular}
    
    \label{tab:res-nlp-corpora}
\end{table}

==> tables/result_aic.tex <==
\begin{table}[h]
    \centering
    \caption{The best design model uses only the story type for the fixed effect. The AIC values for the mixed effect models using the story type or story type and the number of words in the design matrix. The AIC values are relative to the AIC for the model with only the number of words in the design matrix. Smaller the AIC means a better model fit.}
    \begin{tabular}{lcc}
        \toprule
        Parameter & {number of words + story type} & {story type only} \\ \midrule
        no history & 9.90         &   -2.73 \\
        1 sentence history & 10.27        &   -3.69 \\
        2 sentences history & 9.08         &   -3.71 \\
        3 sentences history & 8.29         &   -5.32 \\
        4 sentences history & 7.51         &   -6.14 \\
        5 sentences history & 6.86         &   -7.46 \\
        6 sentences history & 6.97         &   -7.35 \\
        7 sentences history & 7.02         &   -7.45 \\
        8 sentences history & 6.36         &   -8.34 \\
        full history & 6.12         &   -8.87 \\ \bottomrule
    \end{tabular}
    
    \label{tab:sup-aic}
\end{table}
   

